Privacy-Preserving Disclosure and Welfare

We consider a monopolist selling to multiple buyers. A platform observes buyers' tastes and can publicly disclose information about those tastes. However, the platform faces a privacy constraint: the disclosure must reveal nothing about any individual buyer's taste. We show that the same pairs of consumer and producer surplus are attainable with or without this constraint. For each such pair, we construct a privacy-preserving disclosure rule under which a posted-price mechanism attains the pair and no other feasible selling mechanism earns more.

==> references.tex <==
% Shared bibliography for both manuscripts. Keep all entries here; print only
% entries cited in the current document (or explicitly included via \nocite).
\RequirePackage{etoolbox}
\makeatletter
\newcommand{\paper@markcite}[1]{%
  \expandafter\gdef\csname paper@cited@#1\endcsname{}%
}
% natbib builds a normalized list of keys for each citation command.
\apptocmd{\NAT@sort@cites}{%
  \@for\paper@key:=\NAT@cite@list\do{%
    \expandafter\paper@markcite\expandafter{\paper@key}%
  }%
}{}{\PackageError{paper-bibliography}{Could not track natbib citations}{}}
\let\paper@original@nocite\nocite
\renewcommand{\nocite}[1]{%
  \forcsvlist{\paper@markcite}{#1}%
  \paper@original@nocite{#1}%
}
\newcommand{\PaperBibItem}[3][]{%
  \ifcsname paper@cited@*\endcsname
    \bibitem[#1]{#2}#3%
  \else
    \ifcsname paper@cited@#2\endcsname
      \bibitem[#1]{#2}#3%
    \fi
  \fi
}
\makeatother

\newcommand{\PaperBibliography}{%
  \begin{thebibliography}{99}
  \setlength{\itemsep}{0pt}
  \PaperBibItem[Ali, Lewis, and Vasserman(2023)]{AliLewisVasserman2023}{Ali, S. Nageeb, Greg Lewis, and Shoshana Vasserman. 2023. ``Voluntary Disclosure and Personalized Pricing.'' \emph{The Review of Economic Studies} 90(2): 538--571. \url{https://doi.org/10.1093/restud/rdac033}.}

  \PaperBibItem[Banerjee et~al.(2024)Banerjee, Munagala, Shen, and Wang]{BanerjeeMunagalaShenWang2024}{Banerjee, Siddhartha, Kamesh Munagala, Yiheng Shen, and Kangning Wang. 2024. ``Fair Price Discrimination.'' In \emph{Proceedings of the 2024 Annual ACM--SIAM Symposium on Discrete Algorithms (SODA)}, 2679--2703. \url{https://doi.org/10.1137/1.9781611977912.96}.}

  \PaperBibItem[Bergemann, Brooks, and Morris(2015)]{BBM2015}{Bergemann, Dirk, Benjamin Brooks, and Stephen Morris. 2015. ``The Limits of Price Discrimination.'' \emph{American Economic Review} 105(3): 921--957. \url{https://doi.org/10.1257/aer.20130848}.}

  \PaperBibItem[Bergemann and Morris(2019)]{BergemannMorris2019}{Bergemann, Dirk, and Stephen Morris. 2019. ``Information Design: A Unified Perspective.'' \emph{Journal of Economic Literature} 57(1): 44--95. \url{https://doi.org/10.1257/jel.20181489}.}

  \PaperBibItem[Cohen, Elmachtoub, and Lei(2022)]{CohenElmachtoubLei2022}{Cohen, Maxime C., Adam N. Elmachtoub, and Xiao Lei. 2022. ``Price Discrimination with Fairness Constraints.'' \emph{Management Science} 68(12): 8536--8552. \url{https://doi.org/10.1287/mnsc.2022.4317}.}

  \PaperBibItem[Cr\'emer and McLean(1988)]{CremerMcLean1988}{Cr\'emer, Jacques, and Richard P. McLean. 1988. ``Full Extraction of the Surplus in Bayesian and Dominant Strategy Auctions.'' \emph{Econometrica} 56(6): 1247--1257. \url{https://doi.org/10.2307/1913096}.}

  \PaperBibItem[Fallah et~al.(2024)Fallah, Jordan, Makhdoumi, and Malekian]{FallahJordanMakhdoumiMalekian2024}{Fallah, Alireza, Michael I. Jordan, Ali Makhdoumi, and Azarakhsh Malekian. 2024. ``The Limits of Price Discrimination under Privacy Constraints.'' arXiv:2402.08223. \url{https://arxiv.org/abs/2402.08223}.}

  \PaperBibItem[He, Sandomirskiy, and Tamuz(2026)]{HeSandomirskiyTamuz2026}{He, Kevin, Fedor Sandomirskiy, and Omer Tamuz. 2026. ``Private Private Information.'' \emph{Journal of Political Economy} 134(5): 1561--1606. \url{https://doi.org/10.1086/739833}.}

  \PaperBibItem[Ichihashi(2020)]{Ichihashi2020}{Ichihashi, Shota. 2020. ``Online Privacy and Information Disclosure by Consumers.'' \emph{American Economic Review} 110(2): 569--595. \url{https://doi.org/10.1257/aer.20181052}.}

  \PaperBibItem[Ichihashi(2021)]{Ichihashi2021}{Ichihashi, Shota. 2021. ``The Economics of Data Externalities.'' \emph{Journal of Economic Theory} 196: 105316. \url{https://doi.org/10.1016/j.jet.2021.105316}.}

  \PaperBibItem[Ichihashi and Smolin(2025)]{IchihashiSmolin2025}{Ichihashi, Shota, and Alex Smolin. 2025. ``Data Provision to an Informed Seller.'' \emph{Games and Economic Behavior} 153: 131--144. \url{https://doi.org/10.1016/j.geb.2025.06.002}.}

  \PaperBibItem[Kamenica and Gentzkow(2011)]{KamenicaGentzkow2011}{Kamenica, Emir, and Matthew Gentzkow. 2011. ``Bayesian Persuasion.'' \emph{American Economic Review} 101(6): 2590--2615. \url{https://doi.org/10.1257/aer.101.6.2590}.}

  \PaperBibItem[Kr\"ahmer(2020)]{Kraehmer2020}{Kr\"ahmer, Daniel. 2020. ``Information Disclosure and Full Surplus Extraction in Mechanism Design.'' \emph{Journal of Economic Theory} 187: 105020. \url{https://doi.org/10.1016/j.jet.2020.105020}.}

  \PaperBibItem[Kyriazis(2026)]{Kyriazis2026}{Kyriazis, Panagiotis. 2026. ``Shaping the Menu: Information Design under Screening.'' \mbox{arXiv:2610.14225}. \url{https://arxiv.org/abs/2610.14225}.}

  \PaperBibItem[McAfee and Reny(1992)]{McAfeeReny1992}{McAfee, R. Preston, and Philip J. Reny. 1992. ``Correlated Information and Mechanism Design.'' \emph{Econometrica} 60(2): 395--421. \url{https://doi.org/10.2307/2951601}.}

  \PaperBibItem[Munagala, Shen, and Xu(2026)]{MunagalaShenXu2026}{Munagala, Kamesh, Yiheng Shen, and Renzhe Xu. 2026. ``The Limits of Interval-Regulated Price Discrimination.'' In \emph{Web and Internet Economics (WINE 2025)}, Lecture Notes in Computer Science 16266: 90--107. \url{https://doi.org/10.1007/978-3-032-18660-7_6}.}

  \PaperBibItem[Myerson(1981)]{Myerson1981}{Myerson, Roger B. 1981. ``Optimal Auction Design.'' \emph{Mathematics of Operations Research} 6(1): 58--73. \url{https://doi.org/10.1287/moor.6.1.58}.}

  \PaperBibItem[Rassouli, Rosas, and G\"und\"uz(2020)]{RassouliRosasGunduz2020}{Rassouli, Borzoo, Fernando E. Rosas, and Deniz G\"und\"uz. 2020. ``Data Disclosure under Perfect Sample Privacy.'' \emph{IEEE Transactions on Information Forensics and Security} 15: 2012--2025. \url{https://doi.org/10.1109/TIFS.2019.2954652}.}

  \PaperBibItem[Renou and Tomala(2012)]{RenouTomala2012}{Renou, Ludovic, and Tristan Tomala. 2012. ``Mechanism Design and Communication Networks.'' \emph{Theoretical Economics} 7(3): 489--533. \url{https://doi.org/10.3982/TE921}.}

  \PaperBibItem[Roesler and Szentes(2017)]{RoeslerSzentes2017}{Roesler, Anne-Katrin, and Bal\'azs Szentes. 2017. ``Buyer-Optimal Learning and Monopoly Pricing.'' \emph{American Economic Review} 107(7): 2072--2080. \url{https://doi.org/10.1257/aer.20160145}.}

  \PaperBibItem[Shen, Tang, and Zeng(2018)]{ShenTangZeng2018}{Shen, Weiran, Pingzhong Tang, and Yulong Zeng. 2018. ``A Closed-Form Characterization of Buyer Signaling Schemes in Monopoly Pricing.'' In \emph{Proceedings of the 17th International Conference on Autonomous Agents and Multiagent Systems (AAMAS)}, 1531--1539. \url{https://www.ifaamas.org/Proceedings/aamas2018/pdfs/p1531.pdf}.}

  \PaperBibItem[Strack and Yang(2024a)]{StrackYang2024}{Strack, Philipp, and Kai Hao Yang. 2024a. ``Privacy-Preserving Signals.'' \emph{Econometrica} 92(6): 1907--1938. \url{https://doi.org/10.3982/ECTA22017}.}

  \PaperBibItem[Strack and Yang(2024b)]{StrackYangBuyer2024}{Strack, Philipp, and Kai Hao Yang. 2024b. ``Countering Price Discrimination with \mbox{Buyer} Information.'' Working paper. \url{https://www.economics.utoronto.ca/conferences/index.php/cetc/2024/paper/viewFile/1845/497}.}

  \PaperBibItem[Zhu(2023)]{Zhu2023}{Zhu, Shuguang. 2023. ``Private Disclosure with Multiple Agents.'' \emph{Journal of Economic Theory} 212: 105705. \url{https://doi.org/10.1016/j.jet.2023.105705}.}
  \end{thebibliography}
}

